Extrinsic Evaluation of Machine Translation Metrics

Automatic machine translation (MT) metrics are widely used to distinguish the translation qualities of machine translation systems across relatively large test sets (system-level evaluation). However, it is unclear if automatic metrics are reliable at distinguishing good translations from bad translations at the sentence level (segment-level evaluation). In this paper, we investigate how useful MT metrics are at detecting the success of a machine translation component when placed in a larger platform with a downstream task. We evaluate the segment-level performance of the most widely used MT metrics (chrF, COMET, BERTScore, etc.) on three downstream cross-lingual tasks (dialogue state tracking, question answering, and semantic parsing). For each task, we only have access to a monolingual task-specific model. We calculate the correlation between the metric's ability to predict a good/bad translation with the success/failure on the final task for the Translate-Test setup. Our experiments demonstrate that all metrics exhibit negligible correlation with the extrinsic evaluation of the downstream outcomes. We also find that the scores provided by neural metrics are not interpretable mostly because of undefined ranges. We synthesise our analysis into recommendations for future MT metrics to produce labels rather than scores for more informative interaction between machine translation and multilingual language understanding.

==> tables/capitalisation.tex <==
% \begin{table}[]
% \small
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Metrics              & de     & fr    & pt     & es     & zh     \\ \hline
% BLEU          & 0.003  & 0.055 & -0.05  & 0.002  & -0.033 \\
% chrF          & 0.014  & 0.034 & -0.039 & -0.014 & -0.034 \\ \hline
% BERTScore     & 0.013  & 0.039 & -0.009 & -0.005 & -0.037 \\
% COMET-DA      & 0.018  & 0.029 & 0.075  & -0.051 & -0.021 \\ 
% COMET-MQM     & 0.078  & 0.082 & -0.008 & -0.015 & -0.027 \\ 
% UniTE & -0.004 & 0.305 & 0.032  & -0.093 & 0.082  \\ \hline
% \end{tabular}}
% \caption{We report the difference between F1 scores of different metrics for the classification task when the reference is in the (synthetic) truecase v/s lowercase for reference based metrics. The extrinsic task is semantic parsing on the MultiATIS++ dataset where the semantic parser is trained in English. The coloumns report the F1 difference of the respective target language. Casing does not have a conclusive effect on the reference based metrics. $\Delta = truecase - lowercase$}
% \label{tab:capitlisation}
% \end{table}

\begin{table}[t]
\small
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccc@{}} \toprule
Metrics & de & fr & pt & es & zh \\ \midrule
BLEU & 0.003 & 0.055 & -0.050 & 0.002 & -0.033 \\
chrF & 0.014 & 0.034 & -0.039 & -0.014 & -0.034 \\ \midrule
BERTScore & 0.013 & 0.039 & -0.009 & -0.005 & -0.037 \\
COMET-DA & 0.018 & 0.029 & 0.075 & -0.051 & -0.021 \\
COMET-MQM & 0.078 & 0.082 & -0.008 & -0.015 & -0.027 \\
UniTE & -0.004 & 0.305 & 0.032 & -0.093 & 0.082 \\ \bottomrule
\end{tabular}%
}
\caption{Difference between F1 scores of different metrics for the classification task when the reference is in the (synthetic) truecase v/s lowercase for reference based metrics. The extrinsic task is semantic parsing (MultiATIS++SQL) where the semantic parser is trained in English. Columns report the F1 difference of the respective target language. Casing does not have a conclusive effect on the reference based metrics. $\Delta = truecase - lowercase$}
\label{tab:capitlisation}
\end{table}

==> tables/dst_gold_mt.tex <==
% \begin{table}[]
% \resizebox{\linewidth}{!}{

% \begin{tabular}{|c|c|c|c|c|}
% \hline
% Metric \textbackslash Lang & zh     & de     & ar     & ru     \\ \hline
% Good / Bad              & 2542/ 719 & 2876/385 & 2699/562 & 2563/698 \\ \hline
% random                     & 0      & 0.044  & -0.019 & 0.005  \\ \hline
% BLEU                       & 0.067  & 0      & 0.144  & 0.03   \\ \
% chrF                       & -0.058 & 0      & 0      & -0.009 \\ \hline
% BERTScore                  & 0      & 0.012  & -0.02  & 0.048  \\ 
% COMET-DA                   & 0.076  & -0.011 & -0.023 & 0.026  \\ 
% COMET-MQM                  & -0.038 & -0.023 & -0.024 & -0.051 \\ 
% UniTE                      & -0.058 & -0.036 & -0.032 & -0.067 \\ \hline
% COMET-QE                   & -0.058 & -0.024 & -0.04  & -0.048 \\ 
% COMET-QE-MQM               & -0.057 & 0.033  & -0.021 & -0.069 \\ 
% UniTE-QE                   & -0.069 & -0.012 & -0.04  & -0.072 \\ \hline
% \end{tabular}}
% \caption{MCC scores for metrics when extrinsic task is dialogue state tracking when the dialogue history is gold translations and only the context is automatically translated. Number of bad examples decrease compared to Table \ref{tab:dst-main} indicating cascading of errors due to incorrect translations in the dialogue history. Metrics also perform poor than Table \ref{tab:dst-main}.}
% \label{tab:dst-gold}
% \end{table}

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccc@{}}
\toprule
Language & zh & de & ar & ru \\
Good / Bad & 2542/ 719 & 2876/385 & 2699/562 & 2563/698 \\ \midrule
Random & 0.000 & 0.044 & -0.019 & 0.005 \\ \midrule
BLEU & 0.067 & 0.000 & 0.144 & 0.030 \\
chrF & -0.058 & 0.000 & 0.000 & -0.009 \\ \midrule
BERTScore & 0.000 & 0.012 & -0.020 & 0.048 \\
COMET-DA & 0.076 & -0.011 & -0.023 & 0.026 \\
COMET-MQM & -0.038 & -0.023 & -0.024 & -0.051 \\
UniTE & -0.058 & -0.036 & -0.032 & -0.067 \\ \midrule
COMET-QE & -0.058 & -0.024 & -0.040 & -0.048 \\
COMET-QE-MQM & -0.057 & 0.033 & -0.021 & -0.069 \\
UniTE-QE & -0.069 & -0.012 & -0.040 & -0.072 \\ \bottomrule
\end{tabular}%
}
\caption{MCC metric scores for extrinsic Dialogue State Tracking when the dialogue history is gold translations and only the context is automatically translated. Number of bad examples decrease compared to Table \ref{tab:dst-main} indicating cascading of errors due to incorrect translations in the dialogue history. Metrics also perform poor than Table \ref{tab:dst-main}.}
\label{tab:dst-gold}
\end{table}


==> tables/dst_rtt.tex <==
% \begin{table}[]
% \small
% \centering
% \resizebox{\linewidth}{!}{

% \begin{tabular}{|c|c|c|c|c|}
% \hline
% Method    & zh    & de     & ar     & ru     \\ \hline
% %Good / Bad  &   1465 / 1796    &        &        &        \\ \hline
% BLEU      & 0.078 & 0.025 & -0.065 & -0.103 \\
% chrf      & 0.314 & 0.211 & 0.128  & -0.018 \\ \hline
% BERTScore & 0.313 & 0.229 & 0.15   & -0.017 \\
% COMET-DA & 0.158 & 0.14  & 0.075  & -0.105 \\ 
% COMET-MQM & 0.18  & 0.167 & 0      & -0.115 \\ \hline

% \end{tabular}}
% \caption{MCC scores of reference based metrics for the extrinsic task of dialogue state tracking. The setup simulates an online setting where gold standard references are not available. Instead, the translation is translated back into the target language. MCC scores improve in this setup over Table \ref{tab:dst-main} as long as the quality of machine translation is high (zh, de, ar).}
% \label{tab:rtt-dst}
% \end{table}

\begin{table}[t]
\small
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccc@{}}
\toprule
Method & zh & de & ar & ru \\ \midrule
BLEU & 0.078 & 0.025 & -0.065 & -0.103 \\
chrF & 0.314 & 0.211 & 0.128 & -0.018 \\ \midrule
BERTScore & 0.313 & 0.229 & 0.150 & -0.017 \\
COMET-DA & 0.158 & 0.140 & 0.075 & -0.105 \\
COMET-MQM & 0.180 & 0.167 & 0.000 & -0.115 \\ \bottomrule
\end{tabular}%
}
\caption{MCC scores of reference based metrics for the extrinsic Dialogue State Tracking. The setup simulates an online setting without gold standard references. Instead, the translation is translated back into the target language. MCC scores improve in this setup over Table \ref{tab:dst-main} assuming high quality machine translation (zh, de, ar).}
\label{tab:rtt-dst}
\end{table}

==> tables/parsing_de.tex <==
% \begin{table*}[]
% \small
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% Metric / Lang         & \multicolumn{2}{c|}{en}        & \multicolumn{2}{c|}{fr}       & \multicolumn{2}{c|}{pt}        & \multicolumn{2}{c|}{es}        & \multicolumn{2}{c|}{zh}        \\
% Good / Bad & \multicolumn{2}{c|}{220 / 119} & \multicolumn{2}{c|}{293 / 46} & \multicolumn{2}{c|}{210 / 129} & \multicolumn{2}{c|}{193 / 146} & \multicolumn{2}{c|}{174 / 165} \\ \hline
%              & F1    & MCC    & F1    & MCC    & F1    & MCC   & F1    & MCC    & F1    & MCC    \\\hline
% random       & 0.49  & -0.003 & 0.409 & -0.007 & 0.462 & -0.07 & 0.479 & -0.035 & 0.468 & -0.063 \\\hline
% BLEU         & 0.611 & 0.226  & 0.523 & 0.046  & 0.592 & 0.184 & 0.605 & 0.23   & 0.614 & 0.241  \\
% chrF         & 0.598 & 0.21   & 0.539 & 0.078  & 0.641 & 0.3   & 0.621 & 0.242  & 0.67  & 0.34   \\ \hline
% BERTScore    & 0.623 & 0.251  & 0.515 & 0.033  & 0.638 & 0.312 & 0.569 & 0.2    & 0.571 & 0.15   \\ 
% COMET-DA     & 0.624 & 0.263  & 0.595 & 0.196  & 0.684 & 0.394 & 0.666 & 0.332  & 0.614 & 0.242  \\
% COMET-MQM    & 0.637 & 0.328  & 0.613 & 0.226  & 0.683 & 0.406 & 0.631 & 0.264  & 0.553 & 0.124  \\
% UniTE        & 0.629 & 0.303  & 0.608 & 0.243  & 0.619 & 0.302 & 0.684 & 0.37   & 0.458 & -0.076 \\ \hline
% COMET-QE-DA  & 0.556 & 0.161  & 0.592 & 0.185  & 0.645 & 0.331 & 0.596 & 0.206  & 0.524 & 0.054  \\
% COMET-QE-MQM & 0.62  & 0.25   & 0.522 & 0.044  & 0.619 & 0.295 & 0.576 & 0.181  & 0.532 & 0.088  \\
% UniTE-QE     & 0.503 & 0.024  & 0.464 & 0      & 0.556 & 0.132 & 0.631 & 0.279  & 0.327 & 0     \\ \hline
% \end{tabular}
% \caption{Performance of different metrics when the extrinsic task is parsing on the MultiATIS++SQL dataset with the parser trained in German. 
% The good/bad are the number of examples in the respective labels for the classification task. Typically, metrics have negligible correlation with the outcomes of the end task.}
% \label{tab:parsing-de}
% \end{table*}

\begin{table*}[t]
\small
\centering
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
Language & \multicolumn{2}{c}{en} & \multicolumn{2}{c}{fr} & \multicolumn{2}{c}{pt} & \multicolumn{2}{c}{es} & \multicolumn{2}{c}{zh} \\ 
Good / Bad & \multicolumn{2}{c}{220 / 119} & \multicolumn{2}{c}{293 / 46} & \multicolumn{2}{c}{210 / 129} & \multicolumn{2}{c}{193 / 146} & \multicolumn{2}{c}{174 / 165} \\ \midrule
Method & F1 & MCC & F1 & MCC & F1 & MCC & F1 & MCC & F1 & MCC \\ \midrule 
Random & 0.490 & -0.003 & 0.409 & -0.007 & 0.462 & -0.070 & 0.479 & -0.035 & 0.468 & -0.063 \\ \midrule
BLEU & 0.611 & 0.226 & 0.523 & 0.046 & 0.592 & 0.184 & 0.605 & 0.230 & 0.614 & 0.241 \\
chrF & 0.598 & 0.210 & 0.539 & 0.078 & 0.641 & 0.300 & 0.621 & 0.242 & 0.670 & 0.340 \\ \midrule
BERTScore & 0.623 & 0.251 & 0.515 & 0.033 & 0.638 & 0.312 & 0.569 & 0.200 & 0.571 & 0.150 \\
COMET-DA & 0.624 & 0.263 & 0.595 & 0.196 & 0.684 & 0.394 & 0.666 & 0.332 & 0.614 & 0.242 \\
COMET-MQM & 0.637 & 0.328 & 0.613 & 0.226 & 0.683 & 0.406 & 0.631 & 0.264 & 0.553 & 0.124 \\ 
UniTE & 0.629 & 0.303 & 0.608 & 0.243 & 0.619 & 0.302 & 0.684 & 0.370 & 0.458 & -0.076 \\ \midrule
COMET-QE-DA & 0.556 & 0.161 & 0.592 & 0.185 & 0.645 & 0.331 & 0.596 & 0.206 & 0.524 & 0.054 \\
COMET-QE-MQM & 0.620 & 0.250 & 0.522 & 0.044 & 0.619 & 0.295 & 0.576 & 0.181 & 0.532 & 0.088 \\
UniTE-QE & 0.503 & 0.024 & 0.464 & 0.000 & 0.556 & 0.132 & 0.631 & 0.279 & 0.327 & 0.000 \\ \bottomrule
\end{tabular}%
% }
\caption{MT Metric performance for extrinsic semantic parsing (MultiATIS++SQL) with the parser trained in German (de). 
Good/Bad are the number of examples in the respective labels for the classification task. Typically, metrics have negligible correlation with the outcomes of the end task.}
\label{tab:parsing-de}
\end{table*}

==> tables/task-parsing.tex <==
\begin{table}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & EN    & FR    & PT    & ES    & DE    & ZH    \\ \hline
EN                     & 75.59 & 59.62 & 38.03 & 58.92 & 61.03 & 55.16 \\ \hline
FR                     & 46.48 & 72.77 & 54.93 & 38.97 & 68.08 & 13.65 \\ \hline
PT                     & 54.93 & 59.86 & 72.77 & 28.17 & 50.94 & 2.38  \\ \hline
ES                     & 51.88 & 50.47 & 42.49 & 63.68 & 49.30 & 4.74  \\ \hline
DE                     & 50.70 & 67.14 & 47.42 & 43.43 & 75.59 & 40.85 \\ \hline
ZH                     & 44.60 & 37.09 & 24.88 & 12.00 & 32.86 & 72.07 \\ \hline
\end{tabular}
\caption{}
\label{tab:task-parsing}
\end{table}

==> tables/xquad_qs.tex <==
\begin{table*}[t]
\small
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Method / Lang      & ar     & de     & el     & es     & hi     & ru     & th     & tr     & vi     & zh     \\ \hline
Good / Bad & 592 / 264 & 696 / 169 & 701/ 170 & 721 / 152 & 631 / 241 & 701 / 173 & 539 / 323 & 443 / 389 & 616 / 251 & 606 / 266 \\ \hline
random       & 0.023 & -0.002 & -0.002 & 0.017  & 0.001 & -0.002 & -0.002 & 0.028  & -0.051 & -0.045 \\ \hline
BLEU         & 0.179 & 0.1    & 0.155 & 0.131 & 0.144 & 0.139 & 0.183 & 0.178 & 0.23  & 0.209 \\
chrF         & 0.226 & 0.082  & 0.2   & 0.124 & 0.198 & 0.167 & 0.171 & 0.181 & 0.241 & 0.227 \\ \hline
BERTScore    & 0.184 & 0.084  & 0.209 & 0.174 & 0.245 & 0.216 & 0.197 & 0.255 & 0.246 & 0.284 \\
COMET-DA     & 0.283 & 0.151  & 0.252 & 0.142 & 0.222 & 0.236 & 0.194 & 0.233 & 0.219 & 0.23  \\
COMET-MQM    & 0.09  & 0.048  & 0.171 & 0.162 & 0.161 & 0.197 & 0.166 & 0.165 & 0.214 & 0.161 \\
UniTE        & 0.225 & 0.096  & 0.242 & 0.271 & 0.266 & 0.244 & 0.203 & 0.239 & 0.267 & 0.262 \\ \hline
COMET-QE     & 0.131 & 0.067  & 0.165 & 0.108 & 0.059 & 0.114 & 0.097 & 0.189 & 0.146 & 0.083 \\
COMET-QE-MQM & 0.055 & -0.011 & 0     & 0.078 & 0.062 & 0.111 & 0.121 & 0.159 & 0.083 & 0.054 \\
UniTE-QE     & 0.166 & 0.109  & 0.169 & 0.124 & 0.213 & 0.124 & 0.126 & 0.182 & 0.259 & 0.178 \\ \hline
\end{tabular}}
\caption{QA Results}
\label{tab:xquad-qs}
\end{table*}

==> tables/zero_shot.tex <==
% \begin{table}[]
% \small
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% src-tgt                    & en-es  & pt-en     & es-de     & zh-fr  & de-zh     \\ \hline
% examples                 & 193/92 & 171 / 172 & 193 / 196 & 53/275 & 144 / 183 \\ \hline
% random                   & 0.455  & 0.466     & 0.479     & 0.384  & 0.503     \\ \hline
% %BLEU                     & 0.075  & 0.21      & 0.126     & 0.257  & 0.127     \\
% %chrF                     & 0.106  & 0.193     & 0.142     & 0.318  & 0.134     \\ \hline
% %BERTScore       & 0.111  & 0.148     & 0.09      & 0.282  & 0.147     \\
% COMET-DA            & 0.15   & 0.089     & 0.187     & 0.283  & 0.145     \\
% COMET-MQM     & 0.146  & 0.143     & 0.152     & 0.274  & 0.159     \\
% UniTE            & -0.031 & -0.039    & 0.205     & 0.121  & 0.094     \\ \hline
% COMET-QE-DA      & 0.089  & 0.061     & 0.117     & 0.137  & 0.036     \\
% COMET-QE-MQM & 0.109  & 0.118     & 0.097     & 0.118  & 0.053     \\
% UniTE-QE                & -0.022 & 0.065     & 0.152     & 0.194  & 0.014    \\ \hline
% \end{tabular}}
% \caption{Difference of macro F1 scores of different metrics and random baseline with semantic parsing as extrinsic task to check generalisation of metrics . The top row has absolute macro F1 scores for the random baseline and every other row is $\Delta = metric_{F1} - random_{F1}$. The first language in the pair is the source language of the task-specific model. The second language is the target language used in the translate test setting. The metrics show similar yet poor performance to Table \ref{tab:parsing-de}. }
% \label{tab:zero-shot}
% \end{table}

\begin{table}[t]
\small
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccc@{}}
\toprule
src-tgt & en-es & pt-en & es-de & zh-fr & de-zh \\
Examples & 193/92 & 171 / 172 & 193 / 196 & 53/275 & 144 / 183 \\ \midrule
Random & 0.455 & 0.466 & 0.479 & 0.384 & 0.503 \\ \midrule
% BLEU & 0.075 & 0.210 & 0.126 & 0.257 & 0.127 \\
% chrF & 0.106 & 0.193 & 0.142 & 0.318 & 0.134 \\
% BERTScore & 0.111 & 0.148 & 0.09 & 0.282 & 0.147 \\
COMET-DA & 0.150 & 0.089 & 0.187 & 0.283 & 0.145 \\
COMET-MQM & 0.146 & 0.143 & 0.152 & 0.274 & 0.159 \\
UniTE & -0.031 & -0.039 & 0.205 & 0.121 & 0.094 \\ \midrule
COMET-QE-DA & 0.089 & 0.061 & 0.117 & 0.137 & 0.036 \\
COMET-QE-MQM & 0.109 & 0.118 & 0.097 & 0.118 & 0.053 \\
UniTE-QE & -0.022 & 0.065 & 0.152 & 0.194 & 0.014 \\ \bottomrule
\end{tabular}%
}
\caption{Difference of Macro F1 scores of different metrics and random baseline for extrinsic semantic parsing to verify metric generalisation. The lead row has absolute macro F1 scores for the random baseline and every other row is $\Delta = metric_{F1} - random_{F1}$. The first language in the pair is the source language of the task-specific model. The second language is the target language used in the \textit{Translate-Test} setting. The metrics show similar yet poor performance to Table \ref{tab:parsing-de}.}
\label{tab:zero-shot}
\end{table}
